Adaptive Multi-view Rule Discovery for Weakly-Supervised Compatible Products Prediction

On e-commerce platforms, predicting if two products are compatible with each other is an important functionality to achieve trustworthy product recommendation and search experience for consumers. However, accurately predicting product compatibility is difficult due to the heterogeneous product data and the lack of manually curated training data. We study the problem of discovering effective labeling rules that can enable weakly-supervised product compatibility prediction. We develop AMRule, a multi-view rule discovery framework that can (1) adaptively and iteratively discover novel rulers that can complement the current weakly-supervised model to improve compatibility prediction; (2) discover interpretable rules from both structured attribute tables and unstructured product descriptions. AMRule adaptively discovers labeling rules from large-error instances via a boosting-style strategy, the high-quality rules can remedy the current model's weak spots and refine the model iteratively. For rule discovery from structured product attributes, we generate composable high-order rules from decision trees; and for rule discovery from unstructured product descriptions, we generate prompt-based rules from a pre-trained language model. Experiments on 4 real-world datasets show that AMRule outperforms the baselines by 5.98% on average and improves rule quality and rule proposal efficiency.

==> table/rule_example.tex <==
\scalebox{1.0}{
\begin{tabular}{rp{15cm}}\hline
     Input :& Microsoft is an American technology corporation founded by Bill Gates. \\
     Prompt :& \texttt{[Input]} The Person
     {Bill Gates} \texttt{[Mask]} the Organization {Microsoft}.\\
     Rule :& 
     \{Entity Pair $==$ [Person, Org]\} $\land$ \{\texttt{[Mask]} $==$ \textit{founded}\} $\land$ \{$s_{t,j} \geq \text{threshold}$\} $\to$ \textbf{per:found} \\\hline
     Input :&  Marvell Software Solutions Israel is a wholly owned subsidiary of Marvell Technology Group.\\
     Prompt :& \texttt{[Input]} The {Marvell Software Solutions Israel} is a \texttt{[Mask]}.\\
     Rule :& 
     \{\texttt{[Mask]} $==$ \textit{subsidiary $\lor$ corporation $\lor$ company}\} $\land$ \{$s_{t,j} \geq \text{threshold}$\}  $\to$ \textbf{Company}\\\hline
     Input :&  Liverpool short of firepower for crucial encounter. Rafael Benitez must gamble with Liverpools Champions League prospects tonight but lacks the ammunition to make it a fair fight.\\
     Prompt :& \texttt{[Mask]} News: \texttt{[Input]} \\
     Rule :&
     \{\texttt{[Mask]} $==$ \textit{Liverpools $\lor$ Team $\lor$  Football  $\lor$  Sports}\}
     $\land$ \{$s_{t,j} \geq \text{threshold}$\} $\to$ \textbf{Sports} \\\hline
\end{tabular}
}


